Positional Information is All You Need: A Novel Pipeline for Self-Supervised SVDE from Videos

Recently, much attention has been drawn to learning the underlying 3D structures of a scene from monocular videos in a fully self-supervised fashion. One of the most challenging aspects of this task is handling the independently moving objects as they break the rigid-scene assumption. For the first time, we show that pixel positional information can be exploited to learn SVDE (Single View Depth Estimation) from videos. Our proposed moving object (MO) masks, which are induced by shifted positional information (SPI) and referred to as `SPIMO' masks, are very robust and consistently remove the independently moving objects in the scenes, allowing for better learning of SVDE from videos. Additionally, we introduce a new adaptive quantization scheme that assigns the best per-pixel quantization curve for our depth discretization. Finally, we employ existing boosting techniques in a new way to further self-supervise the depth of the moving objects. With these features, our pipeline is robust against moving objects and generalizes well to high-resolution images, even when trained with small patches, yielding state-of-the-art (SOTA) results with almost 8.5x fewer parameters than the previous works that learn from videos. We present extensive experiments on KITTI and CityScapes that show the effectiveness of our method.

==> Tables/table_ablation_param.tex <==
\begin{tabular}{lcccccc}
\hline
Methods & Param & abs rel\cellcolor{c_lowbest} & sq rel\cellcolor{c_lowbest} & rmse\cellcolor{c_lowbest} & rmse$_{log}$\cellcolor{c_lowbest}  & $\delta^1$\cellcolor{c_highbest}  \\ 
\hline
AQUAD-Net-n & 12 & - & - & - & - & - \\
AQUAD-Net   & 15 & - & - & - & - & - \\
AQUAD-Net-w & 30 & - & - & - & - & - \\

\hline
\end{tabular}

==> Tables/table_ablation_s.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{clccccccc}
\hline
Expmt. & Methods & abs rel\cellcolor{c_lowbest} & sq rel\cellcolor{c_lowbest} & rmse\cellcolor{c_lowbest} & rmse$_{log}$\cellcolor{c_lowbest}  & $\delta^1$\cellcolor{c_highbest} & $a^2$\cellcolor{c_highbest} & $a^3$\cellcolor{c_highbest} \\ 
\hline

% \multicolumn{6}{l}{First training stage}\\
1&AQUANet (1st) & 0.120 & 1.457 & 4.286 & 0.167 & 0.891 & 0.970 & 0.986 \\
&AQUANet (1st-stat) & 0.080 & 0.287 & 2.858 & 0.114 & 0.936 & 0.992 & 0.999 \\
\hline

% \multicolumn{6}{l}{Effects of second stage on different architectures}\\
% 2 & vPLADE-Net($1^{st}$) & 0.114 & 1.073 & 4.078 & 0.161 & 0.900 \\ % 0.9737    0.9881 \\
% Kitti\11-15-04_56\DIRnet_inc3_ns0b,e110es,b8,lr1e-05
2 &AQUANet (with \cite{monodepth2} masks) & 0.113 & 0.820 & 4.236 & 0.167 & 0.881 & 0.970 & 0.989 \\
& DIRNet-BW & 0.098 & 0.579 & 3.910 & 0.149 & 0.900 & 0.976 & 0.992 \\
& vPLADE-Net  & 0.084 & 0.366 & 3.240 & 0.124 & 0.930 & 0.987 & 0.997 \\
& AQUANet &  0.080 & 0.328 & 3.095 & 0.118 & 0.934 & 0.989 & 0.997 \\
\hline

% \multicolumn{6}{l}{Effects of special augmentation protocol}\\
3 & AQUANet (no aug.) & 0.098 & 0.532 & 3.923 & 0.146 & 0.902 & 0.978 & 0.993 \\
& AQUANet (inverse)   & 0.091 & 0.417 & 3.446 & 0.131 & 0.918 & 0.986 & 0.996 \\
& AQUANet (invariant) & 0.087 & 0.385 & 3.288 & 0.126 & 0.925 & 0.987 & 0.997 \\
\hline

% \multicolumn{6}{l}{Effects of boosting}\\
4 & AQUANet($a_b=0.1$) & 0.078 & 0.320 & 3.117 & 0.117 & 0.935 & 0.989 & 0.997 \\
&AQUANet(full) & 0.077 & 0.324 & 3.032 & 0.115 & 0.938 & 0.989 & 0.997 \\
\hline

% \multicolumn{6}{l}{Effects of adaptive quantization}\\
5 & AQUANet(per-dataset) & 0.078 & 0.332 & 3.070 & 0.117 & 0.935 & 0.988 & 0.997 \\
&AQUANet(per-image) & 0.085 & 0.362 & 3.373 & 0.128 & 0.921 & 0.985 & 0.997 \\
\hline

\end{tabular}

==> Tables/table_results_kitti.tex <==
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{>{\cellcolor{c_data}}cclcccccccccc}
\hline
& Ref & Methods & Sup & Data & Par & abs rel\cellcolor{c_lowbest}  & sq rel\cellcolor{c_lowbest}  & rmse\cellcolor{c_lowbest}  & log$_{rmse}$\cellcolor{c_lowbest}  & $a^1$\cellcolor{c_highbest} & $a^2$\cellcolor{c_highbest} & $a^3$\cellcolor{c_highbest} \\ 
\cline{2-13}

% Supervised
% Depth of field					
&\cite{singleviewstereo} & Luo \etal & D+S  & K & - & \textbf{0.094} & \textbf{0.626} & \underline{4.252} & \underline{0.177} & \textbf{0.891} & \underline{0.965} & \underline{0.984} \\	
&\cite{defocus} & Gur \etal & DoF & K & - & \underline{0.110} & \underline{0.666} & \textbf{4.186} & \textbf{0.168} & \underline{0.880} & \textbf{0.966} & \textbf{0.988} \\ 
\cline{2-13}

% Self-sup stereo
&\cite{depth_hints}    & DepthHints(P)  & S$_{\text{SGM}}$ & K & 35 & 0.096 & 0.710 & 4.393 & 0.185 & 0.890 & 0.962 & 0.981 \\
&\cite{falnet} & FAL-net & S & K+CS & 17 & \underline{0.091} & \textbf{0.562} & \underline{4.016} & \underline{0.178} & \underline{0.894} & \underline{0.964} & \underline{0.983} \\
&\cite{pladenet} & PLADE-Net & S & K+CS & 15 & \textbf{0.090} & \underline{0.577} & \textbf{3.880} & \textbf{0.170} & \textbf{0.903} & \textbf{0.968} & \textbf{0.985} \\
% &\cite{dbooster} & DBoosterNet-e & & S & K+CS & 14 & \underline{0.087} & \underline{0.553} & \underline{3.891} & \underline{0.169} & \textbf{0.905} & \underline{0.968} & \underline{0.985} \\
\cline{2-13}

% Self-sup video
&\cite{depthwild}    & Gordon \etal & V & K & - & 0.128 & 0.959 & 5.230 & 0.212 & 0.845 & 0.947 & 0.976 \\
&\cite{highresdepth} & Zhou \etal & V & K & 34 & 0.121 & 0.837 & 4.945 & 0.197 & 0.853 & 0.955 & 0.982 \\
&\cite{monodepth2}   & Monodepth2 & V & K & 14 & 0.115 & 0.882 & 4.701 & 0.190 & 0.879 & 0.961 & 0.982 \\	
&\cite{feat_depth}   & FeatDepth & V & K & 73 & \underline{0.104} & 0.729 & 4.481 & \underline{0.179} & 0.893 & \underline{0.965} & \textbf{0.984} \\	
&\cite{packing3d}    & PackNet & V & K & 120 & 0.107 & 0.802 & 4.538 & 0.186 & 0.889 & 0.962 & 0.981 \\
&\cite{hr_depth}   & HR-Depth & V & K & 14 & \underline{0.104} & 0.727 & 4.410 & \underline{0.179} & 0.894 & \textbf{0.966} & \textbf{0.984} \\	
&- & \textit{AQUANet} & V & K & 14 & 0.115 & \textbf{0.656} & \textbf{4.251} & 0.186 & 0.875 & 0.959 & \underline{0.983} \\

&\cite{depthwild}    & Gordon \etal & V & K+CS & - & 0.124 & 0.930 & 5.120 & 0.206 & 0.851 & 0.950 & 0.978 \\
&\cite{sg_depth}   & SG-Depth & V & K+CS & 16 & 0.107 & 0.768 & 4.468 & 0.186 & 0.891 & 0.963 & 0.982 \\	
&\cite{packing3d}    & PackNet & V & CS$\rightarrow$K & 120 & \underline{0.104} & 0.758 & 4.386 & 0.182 & \underline{0.895} & 0.964 & 0.982 \\ 
% \cite{packing3d}    & PackNet & & V+v & CS$\rightarrow$K & 120 & 0.103 & 0.796 & 4.404 & 0.189 & 0.881 & 0.959 & 0.980 \\
&\cite{semguide}     & Guizilini \etal & V+Se & CS$\rightarrow$K & 140 & \textbf{0.100} & 0.761 & 4.270 & \textbf{0.175} & \textbf{0.902} & \underline{0.965} & 0.982 \\
&- & \textit{AQUANet} & V & K+CS & 14 & 0.112 & \underline{0.669} & \underline{4.263} & 0.182 & 0.882 & 0.963 & \textbf{0.984} \\

\cline{2-13}
% &- & \textit{AQUANet} & V & K+DDAD & 14 & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
\multirow{-17}{*}{\rotatebox[origin=c]{90}{Original Eigen Test Split \cite{kitti2012}}}
&- & \textit{AQUANet}(P) & V & K+CS & 14 & 0.110 &  0.637 &   4.170 &   0.179 &   0.885 &    0.964 & 0.984 \\
\hline

% Trained on CS eval on K
% \cite{depthwild}    & Gordon \etal & & V & CS & - & 0.172 & 1.370 & 6.210 & 0.250 & 0.754 & 0.921 & 0.967 \\
% -                 & FAL-netB49   & & S & CS & 17 & \textit{0.144} & \textit{0.871} & \textit{4.796} & \textit{0.215} & \textit{0.811} & \textit{0.947} & \textit{0.979} \\
% \hline

\hline
% Supervised
% \cite{singleviewstereo} & Luo \etal & & DS  & K & - &  \\	
&\cite{vnormal}    & Yin \etal & D & K & 113 & \underline{0.072} & -     & 3.258 & \underline{0.117} & \underline{0.938} & \underline{0.990} & \underline{0.998} \\
&\cite{dorn}       & DORN      & D & K & 51 & 0.072 & 0.307 & \underline{2.727} & 0.120  & 0.932 & 0.984 & 0.995 \\
&\cite{sparse_auxiliary} & PackNet-SAN  & D & K & $>$120 & \textbf{0.052} & \textbf{0.175} & \textbf{2.233} & \textbf{0.083} & \textbf{0.970} & \textbf{0.996} & \textbf{0.999}\\
\cline{2-13}

% Self-sup stereo
&\cite{monodepth2}  & Monodepth2 & V+S & K & 14 & 0.087 & 0.479 & 3.595 & 0.131 & 0.916 & 0.984 & 0.996 \\	
&\cite{depth_hints} & DepthHints(P) & S$_{\text{SGM}}$ & K & 35 & 0.074 & 0.364 & 3.202 & 0.114 & 0.936 & 0.989 & \underline{0.997} \\
&\cite{falnet}  & FAL-net(P) & S & K+CS & 17 & \underline{0.068} & \underline{0.276} & \underline{2.906} & \underline{0.106} & \underline{0.944} & \underline{0.991} & \textbf{0.998} \\
&\cite{pladenet} & PLADE-Net & S & K+CS & 15 & \textbf{0.066} & \textbf{0.263} & \textbf{2.726} & \textbf{0.102} & \textbf{0.949} & \textbf{0.992} & \textbf{0.998} \\
% &\cite{dbooster} & DBoosterNet-e & & S & K+CS & 14 & \underline{0.064} & \underline{0.258} & \underline{2.714} & \underline{0.099} & \underline{0.952} & \underline{0.993} & \textbf{0.998} \\
\cline{2-13}

% Self-sup video
&\cite{monodepth2} & Monodepth2 & V & K & 14 & 0.092 & 0.536 & 3.749 & 0.135 & 0.916 & 0.984 & 0.995 \\
&\cite{packing3d}  & PackNet & V & K & 120 & 0.078 & 0.420 & 3.485 & 0.121 & 0.931 & 0.986 & 0.996 \\
&- & \textit{AQUANet}($1^{st}$) & V & K & 14 & 0.120 & 1.457 & 4.286 & 0.167 & 0.891 & 0.970 & 0.986 \\
% Kitti\09-04-03_07\ADAnet_inc3_ns00f,e110es,b8,lr0.0001
&- & \textit{AQUANet} & V & K & 14 & 0.077 &  \underline{0.324} &  \underline{3.032} & 0.115 & 0.938 & 0.989 & 0.997 \\

&\cite{packing3d}  & PackNet & V+v & CS$\rightarrow$K & 120 & 0.075 & 0.384 & 3.293 & 0.114 & 0.938 & 0.984 & 0.995 \\
&\cite{packing3d}  & PackNet & V & CS$\rightarrow$K & 120 & \textbf{0.071} & 0.359 & 3.153 & \textbf{0.109} & \textbf{0.944} &  \underline{0.990} & \underline{0.997} \\ 
&- & \textit{AQUANet}($1^{st}$) & V & K+CS & 14 & 0.114 & 1.171 & 4.055 & 0.162 & 0.898 & 0.975 & 0.988 \\
% Kitti\09-07-14_27\ADAnet_inc3_ns00f,e110es5600,b8,lr5e-05
&- & \textit{AQUANet} & V & K+CS & 14 &  \underline{0.076} & \textbf{0.301} & \textbf{2.921} &  \underline{0.111} &  \underline{0.943} & \textbf{0.991} & \textbf{0.998} \\

&- & \textit{AQUANet}($1^{st}$) & V & CS & 14 & 0.179 & 1.881 & 5.396 & 0.240 & 0.790 & 0.933 & 0.969 \\
% Cityscapes_video_jpg\08-21-18_08\ADAnet_inc3_ns0f,e110es2900,b4,lr5e-05
&- & \textit{AQUANet} & V & CS & 14 & 0.131 & 0.786 & 4.686 & 0.186 & 0.837 & 0.962 & 0.988 \\ 
\cline{2-13}

                                    % 0.0783    0.3021    2.9096    0.1120    0.9423    0.9910    0.9978
% &- & \textit{AQUANet} &  & V & K+DDAD & 14 & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} & \textbf{} \\
\multirow{-16}{*}{\rotatebox[origin=c]{90}{Improved Test Split \cite{kitti_official}}}
&- & \textit{AQUANet}(P) & V & K+CS & 14 & 0.073 & 0.279 & 2.813 & 0.107 & 0.946 & 0.992 & 0.998 \\

\hline
\end{tabular}
